Of course we share! Testing Assumptions about Social Tagging Systems

Social tagging systems have established themselves as an important part in today's web and have attracted the interest from our research community in a variety of investigations. The overall vision of our community is that simply through interactions with the system, i.e., through tagging and sharing of resources, users would contribute to building useful semantic structures as well as resource indexes using uncontrolled vocabulary not only due to the easy-to-use mechanics. Henceforth, a variety of assumptions about social tagging systems have emerged, yet testing them has been difficult due to the absence of suitable data. In this work we thoroughly investigate three available assumptions - e.g., is a tagging system really social? - by examining live log data gathered from the real-world public social tagging system BibSonomy. Our empirical results indicate that while some of these assumptions hold to a certain extent, other assumptions need to be reflected and viewed in a very critical light. Our observations have implications for the design of future search and other algorithms to better reflect the actual user behavior.

==> data/equality_assumption/categoryCountsTable_old_formatting.tex <==
%%% This file has been created using the class class org.bibsonomy.analysis.tag.CategoryCounting
\begin{tabular}{l|r|r|r}
 & user & resource & tag \\
\hline
\npnoround
\# requests (per entity) & \nprounddigits{2}\numprint{37.96648449698862} & \nprounddigits{2}\numprint{0.14243862959384282} & \nprounddigits{2}\numprint{1.0887658581791455}\\
\hline
\npnoround
\# requests (total) & \npnoround\numprint{680815} & \npnoround\numprint{327703} & \npnoround\numprint{272566}\\
\nprounddigits{2}\# requests (total) & \nprounddigits{2}\numprint{53.14366583299768} & \nprounddigits{2}\numprint{25.58013369927343} & \nprounddigits{2}\numprint{21.27620046772889}\\
\hline
\npnoround
%\# requests (to self) & \npnoround\numprint{567141} & \npnoround\numprint{226903} & \npnoround\numprint{195715}\\
%\nprounddigits{2}
%\% requests (to self) & \nprounddigits{2}\numprint{57.30091870849368} & \nprounddigits{2}\numprint{22.92507570024622} & \nprounddigits{2}\numprint{19.774005591260096}\\
%\hline
%\npnoround
\# requests (to other) & \npnoround\numprint{113674} & \npnoround\numprint{100800} & \npnoround\numprint{76851}\\
%\nprounddigits{2}
\% requests (to other) & \nprounddigits{2}\numprint{39.01965159186476} & \nprounddigits{2}\numprint{34.60053205183215} & \nprounddigits{2}\numprint{26.3798163563031}\\
\end{tabular}
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../../paper"
%%% End:


==> data/equality_assumption/categoryCountsTable_withMySearchBug.tex <==
%%% This file has been created using the class class org.bibsonomy.analysis.tag.CategoryCounting
\begin{tabular}{c|c|c|c}
 & user & resource & tag \\
\hline
\npnoround
\# requests (per entity) & \nprounddigits{2}\numprint{39.93302476020522} & \nprounddigits{2}\numprint{0.14346181380046866} & \nprounddigits{2}\numprint{1.0900041542837056}\\
\hline
\npnoround
\# requests (total) & \npnoround\numprint{716079} & \npnoround\numprint{330057} & \npnoround\numprint{272876}\\
\nprounddigits{2}
\% requests (total) & \nprounddigits{2}\numprint{54.28904361749552} & \nprounddigits{2}\numprint{25.023047553775097} & \nprounddigits{2}\numprint{20.687908828729384}\\
\hline
%\npnoround
%\# requests (to self) & \npnoround\numprint{589892} & \npnoround\numprint{228945} & \npnoround\numprint{196013}\\
%\nprounddigits{2}
%\% requests (to self) & \nprounddigits{2}\numprint{58.12602847711484} & \nprounddigits{2}\numprint{22.55949155047544} & \nprounddigits{2}\numprint{19.314479972409714}\\
%\hline
\npnoround
\# requests (to other) & \npnoround\numprint{126187} & \npnoround\numprint{101112} & \npnoround\numprint{76863}\\
\nprounddigits{2}
\% requests (to other) & \nprounddigits{2}\numprint{41.48677349570295} & \nprounddigits{2}\numprint{33.242811396558416} & \nprounddigits{2}\numprint{25.27041510773864}\\
\end{tabular}
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../../paper"
%%% End:


==> data/equality_assumption/categoryCountsTable_with_autmaticUsers_and_all_status_codes.tex <==
%%% This file has been created using the class class org.bibsonomy.analysis.tag.CategoryCounting
\begin{tabular}{c|c|c|c}
 & user & resource & tag \\
\hline
\npnoround
\# requests (per entity) & \nprounddigits{2}\numprint{39.93302476020522} & \nprounddigits{2}\numprint{0.14346181380046866} & \nprounddigits{2}\numprint{1.0900041542837056}\\
\hline
\npnoround
\# requests (total) & \npnoround\numprint{716079} & \npnoround\numprint{330057} & \npnoround\numprint{272876}\\
\nprounddigits{2}
\% requests (total) & \nprounddigits{2}\numprint{54.28904361749552} & \nprounddigits{2}\numprint{25.023047553775097} & \nprounddigits{2}\numprint{20.687908828729384}\\
%\hline
%\npnoround
%\# requests (to self) & \npnoround\numprint{604952} & \npnoround\numprint{228945} & \npnoround\numprint{196013}\\
%\nprounddigits{2}
%\% requests (to self) & \nprounddigits{2}\numprint{58.738336359487725} & \nprounddigits{2}\numprint{22.229612296220058} & \nprounddigits{2}\numprint{19.03205134429222}\\
\hline
\npnoround
\# requests (to other) & \npnoround\numprint{111127} & \npnoround\numprint{101112} & \npnoround\numprint{76863}\\
\nprounddigits{2}
\% requests (to other) & \nprounddigits{2}\numprint{38.438682541110055} & \nprounddigits{2}\numprint{34.974507267331255} & \nprounddigits{2}\numprint{26.586810191558687}\\
\end{tabular}
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../../paper"
%%% End:


==> data/equality_assumption/equalityTable.tex <==
%%% This file has been created using the class class org.bibsonomy.analysis.tag.CategoryCounting
\begin{tabular}{c|c|c|c}
 & user & resource & tag \\
\hline
\# requests (total) & \numprint{1223830} & \numprint{358325} & \numprint{288085} \\\hline
\% requests (total) & \numprint{65.43705620669004} & \numprint{19.159305757549834} & \numprint{15.403638035760116} \\\hline
\# requests (to other) & \numprint{200790} & \numprint{132991} & \numprint{84115} \\\hline
\% requests (to other) & \numprint{48.04783965388518} & \numprint{31.823946627869134} & \numprint{20.12821371824569} \\\hline
\end{tabular}
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../../paper"
%%% End:


==> tagMakros.tex <==
\newcommand{\pearsonPValue}{\numprint{0.0}} \newcommand{\xOverYKL}{\numprint{0.04696463968425256}} \newcommand{\pearsonCorrelation}{\numprint{0.9923738583314352}} \newcommand{\spearmanCorrelation}{\numprint{0.4385034485705074}} \newcommand{\yOverxKL}{\numprint{0.06406316249325417}} \newcommand{\pearsonError}{\numprint{0.00150400810839295}}

